Data Conflict Resolution Using Trust Mappings

In massively collaborative projects such as scientific or community databases, users often need to agree or disagree on the content of individual data items. On the other hand, trust relationships often exist between users, allowing them to accept or reject other users' beliefs by default. As those trust relationships become complex, however, it becomes difficult to define and compute a consistent snapshot of the conflicting information. Previous solutions to a related problem, the update reconciliation problem, are dependent on the order in which the updates are processed and, therefore, do not guarantee a globally consistent snapshot. This paper proposes the first principled solution to the automatic conflict resolution problem in a community database. Our semantics is based on the certain tuples of all stable models of a logic program. While evaluating stable models in general is well known to be hard, even for very simple logic programs, we show that the conflict resolution problem admits a PTIME solution. To the best of our knowledge, ours is the first PTIME algorithm that allows conflict resolution in a principled way. We further discuss extensions to negative beliefs and prove that some of these extensions are hard. This work is done in the context of the BeliefDB project at the University of Washington, which focuses on the efficient management of conflicts in community databases.

==> conclusions.tex <==
\section{Conclusions}

This paper presents a principled approach to the problem of \emph{conflict resolution} in a \emph{community database} where users \emph{trust} other users with varying priorities. Our semantics has a number of intuitive and desired properties such as independence of the update sequence and, hence, correctly models revoke operations and avoids transient effects. We give a PTIME algorithm that has quadratic worst case scalability in the size of the network. In our experiments, we show that it is actually linear on typical network structures. We also expand our techniques to constraints, and show, depending on the approach taken, conflict resolution can be either intractable, or computable in time that is quadratic in the number of users. In addition, we show how this algorithm can be easily adapted to include bulk processing. 



==> experiments.tex <==
\section{Experiments} \label{sec:experiments}

We have conducted an experimental evaluation of our approach 
addressing the following questions:  What is the observed runtime
performance, both of the quadratic conflict resolution algorithm (RA)
and of the bulk-update algorithm?  And how does our approach compare
to computing the stable models using an advanced liner program solver?  
For the latter we used the programming system DLV
\cite{DBLP:journals/tocl/LeonePFEGPS06}, which is widely considered
the state-of-the-art implementation of logic programming with
negation, and execute it under the brave query
semantics\footnote{command: ``\sql{dlv.bin -brave input.txt
    query.txt}'' }. All algorithms are implemented in Java and were
run on a 2.2GHz dual core machine with 4GB of main
memory. Execution times for RA are averaged over 20 trials.

We used two data sets in our experiments.  The first is a synthetic
data set, consisting of a network of many independent cycles. This
network consists of several, disconnected 4-node clusters of the form
from \specificref{Example}{ex:cycle:cr}. In this network, one out of
two users has an explicit belief.
In our second data set, we modeled a trust network
with as much expected real-life characteristics as possible.
Real-world social structures are known to exhibit a power-law
behavior, often referred to as scale-free.  We used a large crawl of a
top level domain of the World Wide Web and the link structure between
sites which exhibits such behavior, with around 270k domains with 5.4M
links.  We identified domains with users and links with trust
mappings, and assigned random priorities.  We varied the size of
this database by randomly sampling a fraction of all edges and include
both start and end point in our sampled graph.


The results of our experiments are reported in
\autoref{Fig_Experiments}.  For the synthetic data set, as shown
before, DLV runs in exponential time (\autoref{Fig_ExperimentsOscillatorLoop}).  In contrast, RA runs in almost
linear time: thus, just increasing the number of cycles does not lead
to a quadratic running time of our algorithm.  We omit running times
on very small data sets, because they showed high variance due to
factors unrelated to the algorithm (Java memory management, L2 cache
behavior).  \Autoref{Fig_ExperimentsWebData} shows our results on the
real data set.  DLV performs better on this data set, since it
contains fewer cycles, on average. However, our algorithm is still
faster by several orders of magnitude and exhibits the same robust
behavior as before.  Overall, RA had an average running time of around
0.01 msec per user and trust relation on both data sets.

We note that the running time of our algorithm \emph{is} quadratic in
the worst case (we prove this in~\autoref{app:TechnicalReport}), but the types
of graphs that lead to quadratic behavior are complex and highly regular with nested
cycles. We tested our algorithm on such kinds of graphs and measured
running times of about 4 sec for a network size of 10,000.

Finally, \autoref{Fig_ExperimentsBulk} shows our result for testing the
bulk conflict resolution algorithm from~\autoref{sec:bulk}. 
We used a trust network with 7 users and 12 mappings, and assumed two users with
explicit beliefs.  
Then we varied the number of objects in the
database. For each object, we randomly chose these beliefs of the two
users to be in conflict, or in agreement.  Then we reconciled all
users, on all objects.  The database system was Microsoft SQL Server
2005, and we used JDBC for calls to the database.  The data was stored
in a relation $\texttt{POSS(X,K,V)}$, as described in
\autoref{sec:bulk}.  \Autoref{Fig_ExperimentsBulk} shows linear data
scalability of our algorithm\footnote{Data points below 100 msec seem
  to be dominated by the overhead of the Java-SQL server connection}.
The running time of DLV is exponential here too, because of the
conflicts in half of the objects between the two users.  In contrast,
the running time of the bulk conflict resolution algorithm is
independent of the number of conflicts.


\eat{
We illustrate two main characteristics of our approach:
\emph{scalability} and \emph{extendability}. Over a broad range of
realistic network structures our algorithm actually performs in linear
time, and has much potential for further solutions building on it.  At
the same time, we contrast our performance with the best alternative
we could find: calculating the certain or possible tuples with the
answer set programming system DLV
\cite{DBLP:journals/tocl/LeonePFEGPS06}, which is widely considered
the state-of-the-art implementation of logic programming with
negation.  For a given trust network, we generate a LP, such
\specificref{Example}{ex:cycle:cr}, then execute DLV under the brave
query semantics\footnote{command: ``\sql{dlv.bin -brave input.txt
    query.txt}'' }
and record the time it takes to generate all possible tuples. All
algorithms are implemented in Java and are performed on a 2.2GHz dual
core machine with 4G of main memory. Execution times for RA are
averaged over 20 trials.

\introparagraph{Scalability} We focus on one object identifier and
model (i) the trust network structure between users including priority
on edges, (ii) the fraction of explicit beliefs $p_{b_{0}}$, and the
size of the active domain $D$, i.e.\ the number of total conflicting
values. We first consider a network with as many cycles as
possible. This network consists of several, disconnected 4-node
clusters of the form from \specificref{Example}{ex:cycle:cr}. In this
network, one out of two users has an explicit belief, which we
randomly sample from a range of 10 values. As shown before with
\autoref{Fig_DLVexponential}, DLV runs exponentially on this
network. In contrast \specificref{Resolution Algorithm}{alg:bcg} runs
in linear time (\autoref{Fig_ExperimentsOscillatorLoop}). This example
shows that numbers of cycles does not per se force the quadratic
nature of our algorithm.

Second, we try to model a synthetic trust network structure with as
much expected real-life characteristics as possible.  Real-world
social structures are known to exhibit a power-law behavior, often
referred to as scale-free.  We had access to a large crawl of a top
level domain of the World Wide Web and the link structure between
sites which exhibits such behavior.
In our experiments, we take the domains as users and the in-edges as
default mappings and assign the priority of edges randomly.  To show
scalability in size, we randomly sample a fraction of all edges and
include both start and end point in our sampled graph.
\Autoref{Fig_ExperimentsWebData} shows that DLV performs better on
this data set then before since it contains fewer cycles on
average. However, our algorithm is still faster by several orders of
magnitude and exhibits the same robust behavior as before with an
average running time of around 0.01 msec per user and trust
relation. These two experiments suggest that it is robust in a wide
range of network structures.

Third, our algorithm is provably quadratic in the worst case. However,
the network topology must be highly structured with nested cycles and
is not to be expected in real-life data sets. We tested our algorithm
for this case and running time is around 4 sec for a network size of
10,000.


\introparagraph{Extendability} We illustrate the possibilities that
our algorithms allows for further extensions with the bulk insertion
technique sketched in \autoref{sec:bulk}. We use a trust network of
size 19 (7 users and 12 mappings) and assume two users with explicit
beliefs about a varying number of objects in the database. For each
object, we randomly choose these beliefs to be conflicting or in
agreement.  For this experiments we use Microsoft SQL server 2005 and
JDBC for calls to the database, using a schema $\texttt{POSS(X,K,V)}$
for all user relations.  \Autoref{Fig_ExperimentsBulk} shows linear
data scalability of our algorithm\footnote{ Data points below 100 msec
  seem to be dominated by the overhead of the Java-SQL server
  connection} in contrast to the evaluation of the LP.  Also, the high
variance in DLV's running time hints illustrates that DLV is
exponentially affected by the number of conflicts, and hence the
number of possible tuples (see variance of points and trendline). In
contrast, our bulk insertion runs independent of the number of
conflicts.



}



==> relatedWork.tex <==
\section{Related work}

Several systems have been recently described that adopt some kind of \emph{conflict resolution} or \emph{trust mapping} to model data sharing in a community of users
\cite{DBLP:journals/pvldb/GatterbauerBKS09,
DBLP:conf/vldb/GreenKIT07,
DBLP:journals/pvldb/KotK09,
DBLP:conf/sigmod/QiCS07,
DBLP:conf/sigmod/TaylorI06}.
These systems discuss techniques in the presence of various subsets of the features needed in conflict resolution (\autoref{TableWorkComparison}).  Conflicts occur when the system allows key constraints; a conflict is simply a violation of the key constraint.   Orchestra is the only system that considers both conflicts and priorities, and is closest in spirit to our setting.  We share with Youtopia the use of certain/possible values, a concept originally introduced for incomplete databases 
\cite{DBLP:journals/jacm/ImielinskiL84}.




Our solution has relevance to the research areas of \emph{data integration} and \emph{data exchange}.
Similar to~\cite{DBLP:conf/sigmod/TaylorI06}, we assume a fixed schema in this paper. In contrast, work on \emph{peer data exchange} focuses on arbitrary tuple and equality generating dependencies between different database instances with varying schemas.
However, it does not consider priorities amongst different mappings between peers and it is known that data complexity under this semantics is in coNP, and that it can be coNP-complete even for acyclic peer data exchange settings \cite{DBLP:journals/tods/FuxmanKMT06}. 
Those proposals whose semantics is tractable do not consider local integrity constraints (such as key violations) and hence do not model conflicts~\cite{DBLP:journals/pvldb/KotK09}.


Using logic programs and stable models semantics as means to produce certain answers has been proposed before under the framework of \emph{consistent query answering} (CQA) \cite{DBLP:journals/sigmod/Bertossi06}.
However, and as we have illustrated, this approach is generally not tractable;  
no polynomial time case is known for universal constraints with negation \cite[Fig.~1]{DBLP:conf/icdt/Chomicki07}.
As a consequence, previously proposed semantics that build on logic programming 
have coNP data complexity \cite{DBLP:conf/lpar/BertossiB07} and we are not aware of any proposed polynomial algorithm that deals with a principled solution to inconsistency resolution for key constraints and trust mappings.










